ATD: Augmenting CP Tensor Decomposition by Self Supervision

Tensor decompositions are powerful tools for dimensionality reduction and feature interpretation of multidimensional data such as signals. Existing tensor decomposition objectives (e.g., Frobenius norm) are designed for fitting raw data under statistical assumptions, which may not align with downstream classification tasks. In practice, raw input tensors can contain irrelevant information while data augmentation techniques may be used to smooth out class-irrelevant noise in samples. This paper addresses the above challenges by proposing augmented tensor decomposition (ATD), which effectively incorporates data augmentations and self-supervised learning (SSL) to boost downstream classification. To address the non-convexity of the new augmented objective, we develop an iterative method that enables the optimization to follow an alternating least squares (ALS) fashion. We evaluate our proposed ATD on multiple datasets. It can achieve 0.8% - 2.5% accuracy gain over tensor-based baselines. Also, our ATD model shows comparable or better performance (e.g., up to 15% in accuracy) over self-supervised and autoencoder baselines while using less than 5% of learnable parameters of these baseline models

==> relatedwork.tex <==
\section{Related Work}
{\bf Data augmentation and Self-supervised Learning.} Data augmentation exploits class-preserving perturbations to smooth out noise and encode task-invariances \citep{dao2019kernel}. It has been widely used in various data formats, such as images \citep{cirecsan2010deep}, text \citep{lu2006enhancing}, audio \citep{uhlich2017improving}, and time series \citep{wen2020time}. Data augmentation also benefits the recent development of contrastive SSL \citep{he2020momentum,chen2020simple}, which extracts class-relevant features by
optimizing a deep neural network encoder to achieve agreements between semantically similar samples and disagreements 
on dissimilar samples. However, in contrastive SSL, a recent work \cite{arora2019theoretical} highlighted that the common practice of replacing negative samples with random samples leads to sampling bias, which may hurt the learned representation significantly \cite{chuang2020debiased}. In this paper, we introduce an unbiased self-supervised objective into CP tensor decomposition model and shows that the new design can be helpful in producing class-aware outputs.

\smallskip
\noindent{\bf Stochastic Algorithms for Tensors.} With the rapid growth in data volume, efficient stochastic tensor methods become increasingly important for higher-order data structures to boost scalability. These methods are largely based on sampling \citep{ma2021fast,yang2021mtc,kolda2020stochastic}, which accelerates the computation of over-determined least square problems \citep{battaglino2018practical,larsen2020practical} in ALS for dense \citep{ailon2006approximate} and sparse \citep{eshragh2019lsar} tensors by effective strategies, such as Fast Johnson-Lindenstrauss Transform \citep{ailon2006approximate}, leverage-based sampling \citep{eshragh2019lsar}, and sketching. However, these algorithms only focus on making ALS steps less costly and require to load the full data into memory. Thus, we do not consider them in our setting. This paper integrates augmentation techniques and self-supervised loss into tensor decomposition, and later we adopt an effective stochastic alternating optimization to handle large scale optimization with less memory consumption.


